Design of optimization tools for quantum information theory

In this thesis, we present optimization tools for different problems in quantum information theory. First, we introduce an algorithm for quantum estate estimation. The algorithm consists of orthogonal projections on intersecting hyperplanes, which are determined by the probability distributions and the measurement operators. We show its performance, in both runtime and fidelity, considering realistic errors. Second, we present a technique for certifying quantum non-locality. Given a set of bipartite measurement frequencies, this technique finds a Bell inequality that maximizes the gap between the local hidden variable and the quantum value of a Bell inequality. Lastly, to study the quantum marginal problem, we introduce an operator and develop an algorithm, which takes as inputs a set of quantum marginals and eigenvalues, and outputs a density matrix, if exists, compatible with the prescribed data.

==> codigofigura.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[height = 2.5 cm]{core/title_page/logo_HPI.pdf}\\[1 ex]
        \caption{This is the caption of the subfigure that displays the logo of the \textsc{HPI}.}
        \label{fig:HPI}
    \end{subfigure}
    \hfil
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[height = 2.5 cm]{core/title_page/logo_UP.pdf}\\[1 ex]
        \caption{This is the caption of the subfigure that displays the logo of the UP.}
        \label{fig:UP}
    \end{subfigure}
    \caption{These are the two logos featured on the title page. \Cref{fig:HPI} belongs to the HPI, whereas \Cref{fig:UP} belongs to the UP.}
    \label{fig:logos}
\end{figure}


==> conclusions/conclusions.tex <==
% This is where you conclude your thesis.
\epigraph{\itshape La madurez del hombre es haber vuelto a encontrar la seriedad con la que jugaba cuando era niño}{---Friedrich Nietzsche}

\section{Consideraciones finales}

En esta tesis se presentó y estudió una forma plausible para acoplar materia a la teoría de gravedad anisotrópica no--relativista Ho\v{r}ava--Lifshitz. El objetivo central como primer paso en esta dirección, fue establecer de manera coherente el acoplo puro gravedad anisotrópica--campo gauge. 
La validación de tal proceso require que se satisfagan las siguientes condiciones
\begin{enumerate}
    \item Toda solución de la teoría debe respetar una ley de escalamiento anisotrópico entre las coordenadas espaciales y el tiempo.
    \item La teoría resultante debe respetar las simetrías originales, es decir, los difeomorfismos que preservan la foliación.
    \item Se debe preservar el carácter renormalizable por conteo de potencias y la unitaridad. Para ello han de considerarse todos los términos con el máximo de derivadas espaciales que conforman el potencial de interacción tanto del sector gravitacional y gauge, además de garantizar un Hamiltoniano definido positivo.   
\end{enumerate}

Los puntos anteriores son todos provenientes de la propuesta original de Ho\v{r}ava \cite{Horava:2009uw}. En esta dirección, en el presente trabajo de investigación se ha dado una variante posible de como acoplar otras interacciónes a la teoría Ho\v{r}ava--Lifshitz, respetando todas las ideas iniciales. La realización de este objetivo comprendió el análisis detallado de la gravedad anisotrópica Ho\v{r}ava--Lifshitz pura en 4+1 dimensiones \cite{Bellorin:2018wst,Restuccia:2019xdo}, lo cual
sirve como base para el estudio de la teoría en dimensiones más bajas. En general, para la teoría Ho\v{r}ava--Lifshitz formulada en dimensiones arbitrarias se pueden destacar dos aspectos fundamentales:
\begin{enumerate}
    \item El punto crítico de la constante de acoplo $\lambda$ es totalmente dependiente de la dimensión espacial $d$, es decir, $\lambda=1/d$. Por lo tanto, si la teoría en altas dimensiones tiene $d=4$ el valor crítico será $\lambda=1/4$. Esto es de suma importancia, ya que la teoría reducida hereda tal valor.
    \item Al tener $d$--dimensiones espaciales, el número de términos con altas derivadas espaciales compatibles con las simetrías de la teoría incrementa al incrementar $d$. Por lo tanto se espera un mayor número de términos conformando el potencial de la teoría reducida. Además el orden de las derivadas de aquellos objetos también aumenta, recordando que en el caso marginal se incluyen hasta $2z$ derivadas espaciales, con $z=d$.  
\end{enumerate}
Una vez comprendida la teoría 4+1--dimensional en el límite de bajas energías, escala IR, para ambos casos $\lambda$ arbitrario y crítico, se aplicó el esquema de reducción dimensional Kaluza--Klein. Al igual que el protocolo original Kaluza--Klein, se consideró que la dimensión extra está compactificada en un círculo $S^{1}$ y se aplicó la condición cilíndrica. Como consecuencia se obtiene una teoría 3+1--dimensional, concretamente la teoría anisotrópica no--relativista Einstein--Maxwell--dilatón, cuyo grupo de simetrías son los difeomorfismos que preservan la foliación en 3+1--dimensiones y el grupo de transformaciones gauge $U(1)$. El análisis perturbativo revela que esta teoría propaga 6 grados de libertad físicos, 2 asociados al gravitón, 2 al fotón, 1 al dilatón efectivo y 1 al modo de Ho\v{r}ava efectivo, todos no--relativistas. El hecho de decir que el modo de Ho\v{r}ava y el dilatón son modos efectivos, es porque estos grados de libertad están conformados por el escalar de Ho\v{r}ava original más el campo escalar usual que proviene de la reducción dimensional Kaluza--Klein. En contraposición, el caso crítico propaga 5 modos físicos, todos los antes mencionados menos el escalar adicional de Ho\v{r}ava, con lo cual el campo dilatón es el usual. Interesantemente todos estos grados de libertad obedecen ecuaciones hiperbólicas, es decir, ecuaciones de onda, donde el gravitón, el fotón y el dilatón efectivo se propagan a la velocidad $\sqrt{\beta}$, mientras que el modo escalar extra lo hace con una velocidad que compromete también los acoplos $\lambda$ y $\alpha$, lo cual permite restringirlos para evitar cualquier inconsistencia tal como la propagación de campos fantasmas. Para el caso crítico todos los grados de libertad se propagan a la velocidad $\sqrt{\beta}$.

Por otro lado, la obtención del acoplo puro gravedad anisotrópica--campo gauge ocurre cuando desde el inicio se considera que el campo escalar dilatón está en su estado base, es decir, $\Phi=1$ en conjunto con la formulación en el punto crítico. Setear el dilatón en su estado base en la instancia mencionada, se debe a que en etapas posteriores a la reducción dimensional, la teoría se vuelve inconsistente tal como ocurre en las teorías relativistas \cite{Duff:1984hn,Overduin:1998pn}. Esta teoría es la más cercana a la teoría Einstein--Maxwell, ya que propaga ``exactamente'' los mismos grados de libertad físicos, es decir, el gravitón y el fotón, aunque ambos de naturaleza  no--relativista. Un aspecto muy interesante de esta teoría, es la similitud que tiene el sector vectorial con la teoría electromagnética de Maxwell. Ambas comparten la misma estructura a nivel de las ecuaciones de momiento, con la salvedad que el sector gauge anisótropo tiene la presencia de la constante de acoplo $\beta$, la cual al tomar su valor relativista $\beta=1$ reduce las ecuaciones de campo a las ecuaciones de Maxwell. 

Cabe mencionar que bajo ningún punto de vista se ha considerado la teoría en altas dimensiones como la teoría fundamental, siendo la reducida una teoría efectiva. En el punto IR esta interpretación, es decir, considerar la teoría reducida como la fundamental resulta ser inmediata, ya que el espectro que se desprende de la compacficación no depende de las dimensiones extras, ya que se consideran solamente los modos no masivos. Por lo tanto la teoría en altas dimensiones sirve solamente como un marco de partida sin mayor relevancia. Sin embargo, la situación cambia radicalmente en el límite de altas energías, régimen UV. Esto se debe a que el tamaño del radio de compactificación $\varrho$ es del orden de la escala de altas energías, activando así los modos masivos o la denominada torre Kaluza--Klein. Estos modos masivos dependen de las dimensiones extras, lo cual al reducir la teoría hay rastros de la teoría en altas dimensiones. En lo que a esto respecta para el tratamiento cuántico, tal problema se resolvió de la siguiente manera: i) primero de consideró la teoría completa, incluyendo todos los términos hasta orden 8 en derivadas espaciales, compatibles con las simetrías de la teoría. En dicha construcción aparacen contribuciones no triviales del tensor de Weyl \cite{Restuccia:2020nsj}, el cual en la formulación original en 3+1--dimensiones está ausente \cite{Horava:2009uw}. ii) Luego, se realiza la reducción dimensional tomando el límite $\varrho\rightarrow 0$, tal que los modos masivos estén ausentes en la teoría reducida y en consecuencia las dimensiones extras. La teoría reducida 3+1--dimensional completa, contempla absolutamente todos los términos necesarios para la construcción de los propagadores, tanto del sector gravitacional como vectorial. Esto es de suma importancia, ya que la inclusión de todos estos objetos con sus correspondientes constantes de acoplo independientes provienen de la virtud del \emph{approach} Kaluza--Klein, ya que en principio no es posible garantizar la presencia de estos términos si se hubiese partido desde una formulación en 3+1--dimensiones, acoplando cada objeto uno por uno. 

A nivel perturbativo, una vez resueltos los vínculos de primera y segunda clase, se demuestra que hay solamente dos propagadores independientes asociados a los grados de libertad físicos que propaga la teoría, es decir, al gravitón y campo gauge no--relativistas. Ambos propagadores exhiben el mismo comportamiento, a bajas energías o frecuencias son dominados por $\hat{\tilde{g}}_{\kappa}\omega^{2}-\beta\vec{k}^{2}$, mientras que a altas energía o altas frecuencias son dominados por $\hat{\tilde{g}}_{\kappa}\omega^{2}-\beta_{5}\vec{k}^{8}$, lo cual coincide con la idea original de Ho\v{r}ava \cite{Horava:2009uw}. Una característica importante en el estudio cuántico, es que las interacciones no incrementan las potencias de momentum, siendo el máximo orden $2z$, como es requerido para la renormalización por conteo de potencias. En relación a este punto, el grado de divergencia superficial, muestra que la teoría es en efecto renormalizable por conteo de potencias. Además dada la positividad del Hamiltoniano reducido, la teoría es unitaria. En definitiva y como conclusión general de esta investigación, se confirma que la aplicación del esquema Kaluza--Klein dentro del marco de la gravedad Ho\v{r}ava--Lifshitz, es el camino correcto para acoplar campos materiales u otras interacciones a esta teoría de gravedad no--relativista, ya que respeta todos lo lineamientos de la propuesta seminal, es decir, la teoría reducida posee las simetrías originales y se preservan la unitaridad y renormalización por conteo de potencias.  















\section{Problemas abiertos y futuras perspectivas}

El estudio presentado en esta tesis deja algunos problemas abiertos, de los cuales
destacan los siguientes:

\begin{itemize}
    \item Un estudio fenomenológico, que permita acotar los parámetros $\lambda$, $\beta$ y $\alpha$. Esto hará posible la contrastación con las predicciones de Relatividad General y teoría electromagnética de Maxwell.
    \item El estudio de soluciones cosmológicas, que permitan comparar con otras teorías de gravedad modificada en la búsqueda de una explicación a la existencia de los componentes oscuros que abundan en el Universo.
    \item Analizar el comportamiento geodésico y las identidades de Bianchi.
    \item Comparar con teorías relativistas tensoriales--escalares, como la teoría Brans--Dicke. 
    \item Se requiere desarrollar un análisis sistemático de la zona de ondas, para ambos sectores el gravitacional y electromagnético para contrastar con Relatividad General y Maxwell. 
\end{itemize}

==> core/bibliography/bibliography_format.tex <==
% This file contains all of the code that formats the bibliography. Since be package ›biblatex‹ is used, the bibliography needs to be compiled with ›biber‹.
%
% This file contains the following parts:
%   • Resources
%   • Redefined Keywords
%   • Coloring
%   • Format of the Entries
%   • Format of the Own Publications


%\usepackage
%[
%   sortcites,              % Sort multiple references when citing them together.
%    style = numeric,     % alphabetic The style of a citation mark.
%   defernumbers,           % Makes sure that references always have unique numbers. This is important if you use multiple bibliographies.
%  safeinputenc,           % Allows to use UTF8 characters in the bibliography and tries to translate them into TeX automatically.
    %backref = true,         % Creates back references in the bibliography.
%    backrefstyle = three,   % Compresses three or more consecutive pages in the back references into a range.
%    hyperref = true,        % Makes links generated by biblatex clickable. If hyperref is not used, a warning is issued.
%    maxbibnames = 99,       % The maximum number of names displayed in the bibliography.
%    maxcitenames = 2,       % The maximum number of names displayed when using commands like ›textcite‹. The default is 3. After that, ›et al.‹ is used.
%    useprefix,              % Prints name prefixes, such as ›von‹. The default is false. This means that prefixes are not considered to be part of the last name.
%]
%{biblatex} % Used in order to format the bibliography.

%\usepackage[sorting=none]{biblatex}


\usepackage[style=phys, biblabel=brackets, 
backend=biber, 
natbib=true]{biblatex}

% The following command changes the space between the list of authors and the citation mark into a non-breaking space.
\renewcommand\namelabeldelim{\addnbspace}


%%%%%%%%%%%%%%%
%% Resources %%
%%%%%%%%%%%%%%%

\addbibresource{references/strings.bib}                     % Contains many strings for common conference names etc. These strings can then be used in the references.
\addbibresource{references/references.bib}                  % The file that contains the references that are used for the thesis.
%\addbibresource{references/thesis.bib} 

%\addbibresource{references/MyLibrary.bib}                  % The file that contains the references that are used for the thesis.

%\addbibresource{references/Bibliography.bib}                     % Contains many strings for common conference names etc. These strings can then be used in the references.
%\addbibresource{references/references.bib}                  % The file that contains the references that are used for the thesis.


%%%%%%%%%%%%%%%%%%%%%%%%
%% Redefined Keywords %%
%%%%%%%%%%%%%%%%%%%%%%%%

\renewbibmacro{in:}%
{%
    \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}%
}
% \renewcommand*{\volumenumberdelim}{\addcolon}

\renewbibmacro*{volume+number+eid}%
{%
    \printfield{volume}%
    \iffieldundef{number}{}{\addcolon}%
    %  \setunit*{\addnbthinspace}%
    \printfield{number}%
    \setunit*{\addcomma\space}%
    \printfield{eid}%
}

\DefineBibliographyStrings{english}%
{%
    backrefpage  = {\lowercase{s}ee page}, % For a single page number.
   backrefpages = {\lowercase{s}ee pages} % For multiple page numbers.
}


%%%%%%%%%%%%%%
%% Coloring %%
%%%%%%%%%%%%%%

\DeclareFieldFormat[article]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[inproceedings]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[thesis]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[book]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[unpublished]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[report]{title}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[inbook]{chapter}{\textbf{\color{stroke1}#1}}
\DeclareFieldFormat[inbook]{title}{#1}
\DeclareFieldFormat{pages}{#1}


%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Format of the Entries %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The following toggle defines how the citation mark formats the author names. If this toggle is true, more information is used.
\newtoggle{authorend}
\togglefalse{authorend}

% Article
\DeclareBibliographyDriver{article}%
{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \iftoggle{authorend}{}{\usebibmacro{author/translator+others}}%
  \setunit{\labelnamepunct}\newblock
  \usebibmacro{title}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \usebibmacro{bytranslator+others}%
  \newunit\newblock
  \printfield{version}%
  \newunit\newblock
  \usebibmacro{in:}%
  \usebibmacro{journal+issuetitle}%
  \newunit
  \usebibmacro{byeditor+others}%
  \newunit
  \usebibmacro{note+pages}%
  \newunit\newblock
  \iftoggle{bbx:isbn}
  {\printfield{issn}}
  {}%
  \newunit\newblock
  \usebibmacro{doi+eprint+url}%
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \setunit{\bibpagerefpunct}\newblock
 % \usebibmacro{pageref}%
  \newunit\newblock
  \iftoggle{bbx:related}
  {\usebibmacro{related:init}%
    \usebibmacro{related}}
  {}%
  \usebibmacro{finentry}%
  \iftoggle{authorend}{\usebibmacro{author/translator+others}}{}%
}

% Book Chapter
\DeclareBibliographyDriver{inbook}%
{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \iftoggle{authorend}{}{\usebibmacro{author/translator+others}}%
  \setunit{\labelnamepunct}\newblock
  % \usebibmacro{title}%
  \usebibmacro{chapter+pages}%
  % \printfield{chapter}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \usebibmacro{in:}%
  \usebibmacro{bybookauthor}%
  \newunit\newblock
  \usebibmacro{maintitle+booktitle}%
  \newunit\newblock
  \usebibmacro{byeditor+others}%
  \newunit\newblock
  \printfield{edition}%
  \newunit
  \iffieldundef{maintitle}
  {\printfield{volume}%
    \printfield{part}}
  {}%
  \newunit
  \printfield{volumes}%
  \newunit\newblock
  \usebibmacro{series+number}%
  \newunit\newblock
  \printfield{note}%
  \newunit\newblock
  \usebibmacro{publisher+location+date}%
  \newunit\newblock
  % \usebibmacro{chapter+pages}%
  \newunit\newblock
  \iftoggle{bbx:isbn}
  {\printfield{isbn}}
  {}%
  \newunit\newblock
  \usebibmacro{doi+eprint+url}%
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \setunit{\bibpagerefpunct}\newblock
  %\usebibmacro{pageref}%
  \newunit\newblock
  \iftoggle{bbx:related}
  {\usebibmacro{related:init}%
    \usebibmacro{related}}
  {}%
  \usebibmacro{finentry}%
  \iftoggle{authorend}{\usebibmacro{author/translator+others}}{}%
}

% Proceedings Article
\DeclareBibliographyDriver{inproceedings}%
{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \iftoggle{authorend}{}{\usebibmacro{author/translator+others}}%
  \setunit{\labelnamepunct}\newblock
  \usebibmacro{title}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \usebibmacro{in:}%
  \usebibmacro{maintitle+booktitle}%
  \newunit\newblock
  \usebibmacro{event+venue+date}%
  \newunit\newblock
  \usebibmacro{byeditor+others}%
  \newunit\newblock
  \iffieldundef{maintitle}
  {\printfield{volume}%
    \printfield{part}}
  {}%
  \newunit
  \printfield{volumes}%
  \newunit\newblock
  \usebibmacro{series+number}%
  \newunit\newblock
  \printfield{note}%
  \newunit\newblock
  \printlist{organization}%
  \newunit
  \usebibmacro{publisher+location+date}%
  \newunit\newblock
  \usebibmacro{chapter+pages}%
  \newunit\newblock
  \iftoggle{bbx:isbn}
  {\printfield{isbn}}
  {}%
  \newunit\newblock
  \usebibmacro{doi+eprint+url}%
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \setunit{\bibpagerefpunct}\newblock
  %\usebibmacro{pageref}%
  \newunit\newblock
  \iftoggle{bbx:related}
  {\usebibmacro{related:init}%
    \usebibmacro{related}}
  {}%
  \usebibmacro{finentry}%
  \iftoggle{authorend}{\usebibmacro{author/translator+others}}{}%
}

% Thesis
\DeclareBibliographyDriver{thesis}%
{%
  \usebibmacro{bibindex}%
  \usebibmacro{begentry}%
  \iftoggle{authorend}{}{\usebibmacro{author}}%
  \setunit{\labelnamepunct}\newblock
  \usebibmacro{title}%
  \newunit
  \printlist{language}%
  \newunit\newblock
  \usebibmacro{byauthor}%
  \newunit\newblock
  \printfield{note}%
  \newunit\newblock
  \printfield{type}%
  \newunit
  \usebibmacro{institution+location+date}%
  \newunit\newblock
  \usebibmacro{chapter+pages}%
  \newunit
  \printfield{pagetotal}%
  \newunit\newblock
  \iftoggle{bbx:isbn}
  {\printfield{isbn}}
  {}%
  \newunit\newblock
  \usebibmacro{doi+eprint+url}%
  \newunit\newblock
  \usebibmacro{addendum+pubstate}%
  \setunit{\bibpagerefpunct}\newblock
  %\usebibmacro{pageref}%
  \newunit\newblock
  \iftoggle{bbx:related}
  {\usebibmacro{related:init}%
    \usebibmacro{related}}
  {}%
  \usebibmacro{finentry}%
  \iftoggle{authorend}{\usebibmacro{author}}{}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Format of the Own Publications %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The own publications are formatted using a numeric list, whereas the bibliography of the thesis uses an alphanumeric style.

% Copied from numeric.cbx in order to imitate numerical citations.
\providebool{bbx:subentry}
\newbibmacro*{citenum}%
{% Note: the original macro was called ›cite‹. I did not redefine ›cite‹ but instead defined a new macro ›citenum‹ because the author-year citations use the ›cite‹ macro too. Using ›\renewbibmacro*{cite}‹ would have caused all the author-year citations to become numeric too.
  \printtext[bibhyperref]{% If you ever want to use hyperref.
    \printfield{prefixnumber}%
    \printfield{labelnumber}%
    \ifbool{bbx:subentry}
    {\printfield{entrysetcount}}
    {}}%
}

% Copied from numeric.cbx to define a new numeric citation command for @online entries.
\DeclareCiteCommand{\conline}[\mkbibbrackets]
{\usebibmacro{prenote}}
{\usebibmacro{citeindex}%
  \usebibmacro{citenum}}% Note: this was originally "cite" but I changed it to "citenum" to avoid clashes with the author-year style.
{\multicitedelim}
{\usebibmacro{postnote}}

==> core/declaration_of_authorship/declaration_of_authorship.tex <==
I hereby declare that this thesis is my own unaided work. All direct or indirect sources used are acknowledged as references.\\[6 ex]

\begin{flushleft}
    Potsdam, \today
    \hspace*{2 em}
    \raisebox{-0.9\baselineskip}
    {
        \begin{tabular}{p{5 cm}}
            \hline
            \centering\footnotesize\printAuthor
        \end{tabular}
    }
\end{flushleft}

==> introduction/app1.tex <==
\begin{lstlisting}[language=Python, basicstyle=\scriptsize]

import numpy as np
from scipy.optimize import minimize
from scipy.optimize import NonlinearConstraint
import matplotlib.pyplot as plt
import os
import itertools

from datetime import datetime
cwd = os.getcwd()


def optimal_value(filename, m, num_of_outcomes, num_of_trials, marginals_A, 
                  marginals_B, disp = False, save = False):
    
    """
    This routine optimizes R 
    
    Arguments:
    m: number of settings.
    filename: Name of the file where the experimental data is stored.
    marginals_A: a list containing the marginals (expressions like A_i x I ) in the Alice's side that 
                 have to be considered for the calculations.
    marginals_B: a list containing the marginals (expressions like  I x B_i ) in the Bob's side that 
                 have to be considered for the calculations.
    disp: 'True' for displaying the partial results.
    save: 'True' to save the coefficients S, Sax and Sby as numpy tensors in the 'npy_data' folder.
                         
    Returns: 
    Tensors "S", "Sax" and "Sby" containing the coefficients 
    """
    
    foundResults = {}
    SolutionFound = False
    dir1 = ( cwd + '\\npy_data\\' + 's_' + 
        filename + datetime.today().strftime('_%Y-%m-%d') )
    dir2 = ( cwd + '\\npy_data\\' + 'sax_' + 
        filename + datetime.today().strftime('_%Y-%m-%d') )
    dir3 = ( cwd + '\\npy_data\\' + 'sby_' + 
        filename + datetime.today().strftime('_%Y-%m-%d') )
    
    print('n: number of iterations')
    print(60*'_')
    print(f'    n       R         Q         C         \u0394Q         Gap')
    print(60*'_')
    p, c, _ = load_data(filename, m, num_of_outcomes, 
                        marginals_A, marginals_B)
    # initial guess for the optimizer
    s0, bounds = initial_guess(m, num_of_outcomes, marginals_A, marginals_B) 
    n, target = 1, -1
    
    # constraints
    nlc = NonlinearConstraint( lambda x: -target + R( x, p, c, m, num_of_outcomes, marginals_A, marginals_B), 
                              -np.inf, -target ) 

    while n <= num_of_trials:
        res = minimize( R , s0 ,  args=(p, c, m, num_of_outcomes, marginals_A, marginals_B), 
                        method='SLSQP', tol = 1e-20, 
                        options={ 'ftol':1e-20, 'maxiter':5000, 'disp': False}, 
                        bounds=bounds, constraints=[nlc]) 
        # average between the target guess 's0' and the current solution
        # R = -res.fun. Thus, 'res.fun < target' => 'R > -target'
        s0 = (res.x + s0)/2  
                             
        if  res.fun < target:
            SolutionFound = True
            # keeps the solution that satisfies the constraints
            solution = res 
            # updates the target to the best R value found so far
            target = res.fun  
            nlc = NonlinearConstraint( lambda x: -target  
                                      + R( x, p, c, m, num_of_outcomes, marginals_A, marginals_B), 
                                      -np.inf, -target ) # update the constraints
            Q, C, Dq, gap = results( solution.x, p, c, m, 
                                    num_of_outcomes, marginals_A, marginals_B)
            s, sax, sby = vector_to_tensor(solution.x, p, m, num_of_outcomes, marginals_A, marginals_B)
            # save solutions at the 'npy_data' folder
            if save:
                np.save(dir1, s)
                np.save(dir2, sax)
                np.save(dir3, sby)
            # display results
            if disp:
                print( "%5d    %4.5f   %4.5f   %4.5f    %4.5f    %4.5f" 
                      %(n, -solution.fun, Q, C, Dq, gap) )    
        n += 1
    
    if SolutionFound:
        foundResults['Coefficients'] = (s, sax, sby)
        foundResults['values'] = (Q, C, Dq, gap)
        return foundResults
    else:
        print("\nNo solution has been found ...")
    

    
def probs_local_hidden_model(num_of_outcomes , m):
    
    outcomes = [1] + [0 for i in range(num_of_outcomes-1)]
    rows = ( list(i) for i in set( itertools.permutations(outcomes)) )
    
    for i in itertools.product(rows, repeat = m):
        yield np.array(i).T 

        
def lhv_value(s, m, num_of_outcomes ):
    """
    Inputs:
    s: tuple containing the tensors (S, Sax, Sby)
    num_of_outcomes: number of outcomes
    m: number of settings
    
    Returns: 
    local bound for a 2-party scenario, with "m" settings and "num_of_outcomes" possible outcomes
    """
    s, sax, sby = s
    Cmax = -1e10
    for pax in probs_local_hidden_model(num_of_outcomes , m):
        for pby in probs_local_hidden_model(num_of_outcomes , m):
            C =  ( np.sum(sax*pax) + np.sum(sby*pby)  
                  + np.sum( s*np.einsum('ax,by->abxy', pax,pby) ) )
            if C > Cmax:
                Cmax = C
    return Cmax


def quantum_max_violation(s, p):
    """
    Inputs:
    s: tuple containing the tensors (S, Sax, Sby)
    p: tuple containing the tensors (p, pax, pby)
    
    Returns:
    Quantum Value
    """
    s, sax, sby = s
    p, pax, pby = p
    return np.sum(sax*pax) + np.sum(sby*pby) + np.sum(s*p)


def error_quantum_value( s, c, m, num_of_outcomes):
    """
    This function computes the experimental error of the quantum value "Q" from the countings.
    
    Arguments:
    s: tuple containing the tensors (S, Sax, Sby)
    c: a numpy ndarray c[a,b,x,y], containing the experimental countings c(ab|xy)
    m: number of settings 
    num_of_outcomes: number of outcomes
    marginals_A: a list containing the marginals (expressions like A_i x I ) in the Alice's side that 
                 have to be considered for the calculations.
    marginals_B: a list containing the marginals (expressions like  I x B_i ) in the Bob's side that 
                 have to be considered for the calculations.
                 
    Returns:
    experimental error
    
    """
    c,cax,cby = c
    s,sax,sby = s
    Delta_Q, Delta_Q1, Delta_Q2 =  0, 0, 0
    for i in itertools.product(range(m), repeat = 2):
        for l in itertools.product(range(num_of_outcomes), repeat = 2):
            x,y = i
            a,b = l
            dQ = ( s[a,b,x,y]*np.sum( c[:, :, x, y] ) 
                  - np.sum(s[:,:,x,y]*c[:,:,x,y] ) )/( np.sum( c[:, :, x, y] )**2 )
            if False:
                dQ1 = ( sax[a,x]*np.sum( cax[:,x] ) 
                       - np.sum(sax[:,x]*cax[:,x] ) )/( np.sum( cax[:,x] )**2 )
                dQ2 = ( sby[b,y]*np.sum( cby[:,y] ) 
                       - np.sum(sby[:,y]*cby[:,y] ) )/( np.sum( cby[:,y] )**2 )
                Delta_Q1 += dQ1**2*cax[a,x]
                Delta_Q2 += dQ2**2*cby[b,y]
            else:
                dQ = dQ + (1/m)*(  sax[a,x]*np.sum(c[:, :, y,x] ) 
                                 - np.sum(sax[:,x]*c[:,:,x,y]) )/( np.sum( c[:, :, x, y] )**2 )
                dQ = dQ + (1/m)*(  sby[b,y]*np.sum(c[:, :, y,x] ) 
                                 - np.sum(sby[:,y]*c[:,:,x,y]) )/( np.sum( c[:, :, x, y] )**2 )
            Delta_Q += dQ**2*c[a,b,x,y]
            
    return np.sqrt( Delta_Q  + Delta_Q1 + Delta_Q2 )



def initial_guess(m, num_of_outcomes, marginals_A, marginals_B):    
    """
    This function returns the initial guess and the bounds to be used for the optimizer
    
    Inputs:
    num_of_outcomes: number of outcomes
    m: number of settings
    marginals_A: a list containing the marginals (expressions like A_i x I ) in the Alice's side that 
                 have to be considered for the calculations.
    marginals_B: a list containing the marginals (expressions like  I x B_i ) in the Bob's side that 
                 have to be considered for the calculations.
    
    Returns:
    s0: a numpy array with the initial guess
    bounds: a numpy array with the bounds
    """
    nop = (num_of_outcomes**2)*(m**2) + num_of_outcomes**2*(len(marginals_A) + len(marginals_B))
    lb, ub = -1, 1
    bounds =  tuple( [(lb, ub) for i in range(nop)] )
    s0 = np.array(  [(ub - lb) * np.random.random() + lb   for i in range(nop)] )
    
    return s0, bounds


def R( s, p, c, m, num_of_outcomes, marginals_A, marginals_B):
    """
    inputs:
    s: a numpy 1D array
    p: tuple containing the tensors (p, pax, pby)
    c: a tensor c[a,b,x,y], containing the experimental countings c(ab|xy)
    m: number of settings 
    num_of_outcomes: number of outcomes
    marginals_A: a list containing the marginals (expressions like A_i x I ) in the Alice's side that 
                 have to be considered for the calculations.
    marginals_B: a list containing the marginals (expressions like  I x B_i ) in the Bob's side that 
                 have to be considered for the calculations.
    
    Returns:
    - R
    """
    k = (num_of_outcomes**2)*(m**2)
    s = vector_to_tensor(s, p, m, num_of_outcomes, marginals_A, marginals_B)
    Q = quantum_max_violation(s, p)
    C = lhv_value(s, m, num_of_outcomes )
    Dq = error_quantum_value( s, c, m, num_of_outcomes)
    
    return  -(Q - Dq + k)/(C + k)


def vector_to_tensor(s, p, m, num_of_outcomes, marginals_A, marginals_B):
    """
    inputs:
    s: a numpy 1D array
    p: tuple containing the tensors (p, pax, pby)
    m: number of settings 
    num_of_outcomes: number of outcomes
    marginals_A: a list containing the marginals (expressions like A_i x I ) in the Alice's side that 
                 have to be considered for the calculations.
    marginals_B: a list containing the marginals (expressions like  I x B_i ) in the Bob's side that 
                 have to be considered for the calculations.
    
    Returns:
    Tensors (S, Sax, Sby)
    """
    o = num_of_outcomes
    n = m**2*o**2
    sax, sby = np.zeros((2,m)), np.zeros((2,m))
    s, s_marginals = np.array( s[:n] ).reshape((o,o,m,m)),  s[n:]
    
    j = 0
    if len(marginals_A) > 0:
        for x in marginals_A:
            for a in range(o):
                sax[a,x] = s_marginals[j]
                j += 1
    if len(marginals_B) > 0:
        for y in marginals_B:
            for b in range(o):
                sby[b,y] = s_marginals[j]
                j += 1
    s[np.nonzero(p[0] == 0)] = np.zeros((s[np.nonzero(p[0] == 0)].shape[0]))
    
    return (s, sax, sby)



def results( s, p, c, m, num_of_outcomes, marginals_A, marginals_B):
    """
    inputs:
    s: a numpy 1D array
    p: tuple containing the tensors (p, pax, pby)
    c: a tensor c[a,b,x,y], containing the experimental countings c(ab|xy)
    m: number of settings 
    marginals_A: a list containing the marginals (expressions like A_i x I ) in the Alice's side that 
                 have to be considered for the calculations.
    marginals_B: a list containing the marginals (expressions like  I x B_i ) in the Bob's side that 
                 have to be considered for the calculations.
    
    Returns:
    A tuple: (Q, C, DeltaQ, Q - DeltaQ - C)
    """
    o = num_of_outcomes
    n = m**2*o**2
    sax, sby = np.zeros((2,m)), np.zeros((2,m))
    s, s_marginals = np.array( s[:n] ).reshape((o,o,m,m)),  s[n:]
    
    j = 0
    if len(marginals_A) > 0:
        for x in marginals_A:
            for a in range(o):
                sax[a,x] = s_marginals[j]
                j += 1
    if len(marginals_B) > 0:
        for y in marginals_B:
            for b in range(o):
                sby[b,y] = s_marginals[j]
                j += 1
    
    s[np.nonzero(p[0] == 0)] = np.zeros((s[np.nonzero(p[0] == 0)].shape[0]))
    s = (s, sax, sby)
    Q = quantum_max_violation(s, p)
    C = lhv_value(s, m, o )
    Dq = error_quantum_value( s, c, m, o)
    
    return  Q, C, Dq, (Q - Dq - C)



def load_data(name_of_file, m, num_of_outcomes, marginals_A, marginals_B):
    """
    Load the experimental countings saved in "countings_C[C].txt". The file is located in the "experimental_data" folder.
    Each file consists of two columns: 
    1) The labels "abxy" 
    2) the countings c(ab|xy)
    where "a" and "b" are the labels for the outputs of the "x" and "y" settings, respectively.
    Once the countings are loaded, the experimental frecuencies (probabilities) p(ab|xy) are computed.
    
    Inputs:
    filename: Name of the file where the experimental data is stored.
    m: number of settings
    num_of_outcomes: number of outcomes
    marginals_A: a list containing the marginals (expressions like A_i x I ) in the Alice's side that 
                 have to be considered for the calculations.
    marginals_B: a list containing the marginals (expressions like  I x B_i ) in the Bob's side that 
                 have to be considered for the calculations.
    
    Returns:
    p: tuple containing the tensors (p, pax, pby)
    c: a numpy ndarray c[a,b,x,y] containing the countings
       p[a,b,x,y] contains the experimental frecuencies (probabilities).
    measured_marginals: A boolean, which is set to "True" if there are marginal 
                        probabilities in the "countings_C[C].txt" file. 
    
    """
    
    filename = cwd + '\\experimental_data\\' + name_of_file + '.txt'
    
    with open(filename,'r') as f:
        data = f.read()

    data = data.split('\n')
    labels_counts, counts = [] , []
    for i in range(len(data)):
        x,y = tuple( data[i].split()) 
        labels_counts.append(x)
        counts.append(float(y))
    
    countings = dict(zip(labels_counts, counts))
    
    
    shape = (num_of_outcomes,)*2 + (m,)*2 
    p = np.zeros( shape )
    c = np.zeros( shape )
    pax, cax =  np.zeros( (2,2) ), np.zeros( ( 2,2) )
    pby, cby =  np.zeros( (2,2) ), np.zeros( ( 2,2) )
    
    measured_marginals = False
    for l in labels_counts:
        a,b,x,y = l
        if a == '-':
            measured_marginals = True
            cax[int(a),int(x)] = countings[l]
        elif b == '-':   
            measured_marginals = True
            cby[int(b),int(y)] = countings[l]
        else:
            a,b,x,y = list( map( int,l ) )
            c[a,b,x,y] = countings[l]

    for l in labels_counts:
        a,b,x,y = l
        a,b,x,y = list( map( int,l ) )
        if measured_marginals:
            pax[int(a), int(x)] = cax[int(a), int(x)]/( np.sum( cax[:,int(x)] ) )
            pby[int(b), int(y)] = cby[int(b), int(y)]/( np.sum( cby[:,int(y)] ) )
        p[a,b,x,y] = c[a,b,x,y]/( np.sum( c[:,:,x,y] ) )
    
    if len(marginals_A) > 0:
        for x in marginals_A:
            for a in range(2):
                pax[a,x] = np.sum(p[a,: ,x ,0])
    if len(marginals_B) > 0:
        for y in marginals_B:
            for b in range(2):
                pby[b,y] = np.sum(p[:,b ,0 ,y])
    
    return (p, pax, pby) , ( c, cax, cby ), measured_marginals
\end{lstlisting}

    
